Channel Estimation based on Gaussian Mixture Models with Structured Covariances

In this work, we propose variations of a Gaussian mixture model (GMM) based channel estimator that was recently proven to be asymptotically optimal in the minimum mean square error (MMSE) sense. We account for the need of low computational complexity in the online estimation and low cost for training and storage in practical applications. To this end, we discuss modifications of the underlying expectation-maximization (EM) algorithm, which is needed to fit the parameters of the GMM, to allow for structurally constrained covariances. Further, we investigate splitting the 2D time and frequency estimation problem in wideband systems into cascaded 1D estimations with the help of the GMM. The proposed cascaded GMM approach drastically reduces the complexity and memory requirements. We observe that due to the training on realistic channel data, the proposed GMM estimators seem to inherently perform a trade-off between saving complexity/parameters and estimation performance. We compare these low-complexity approaches to a practical and low cost method that relies on the power delay profile (PDP) and the Doppler spectrum (DS). We argue that, with the training on scenario-specific data from the environment, these practical baselines are outperformed by far with equal estimation complexity.

==> graphic.tex <==
% !TeX root = ./WSA21.tex

\resizebox{0.475\textwidth}{!}{%

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt       

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Curve Lines [id:da6463187973732616] 
\draw    (383,112) .. controls (348.35,132.79) and (333.3,87.91) .. (287.4,87.01) ;
\draw [shift={(286,87)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp24515175245695264] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.3 ] (232,170) .. controls (232,165.58) and (235.58,162) .. (240,162) -- (270,162) .. controls (274.42,162) and (278,165.58) .. (278,170) -- (278,194) .. controls (278,198.42) and (274.42,202) .. (270,202) -- (240,202) .. controls (235.58,202) and (232,198.42) .. (232,194) -- cycle ;
%Straight Lines [id:da43670138328003816] 
\draw    (255,117) -- (255,148) ;
\draw [shift={(255,150)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp13195195497504164] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=0.3 ] (79,73) .. controls (79,68.58) and (82.58,65) .. (87,65) -- (117,65) .. controls (121.42,65) and (125,68.58) .. (125,73) -- (125,97) .. controls (125,101.42) and (121.42,105) .. (117,105) -- (87,105) .. controls (82.58,105) and (79,101.42) .. (79,97) -- cycle ;
%Straight Lines [id:da03883995062390988] 
\draw    (222,87) -- (140,87) ;
\draw [shift={(138,87)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp33374729004828074] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ] (354,221.4) .. controls (354,217.87) and (356.87,215) .. (360.4,215) -- (379.6,215) .. controls (383.13,215) and (386,217.87) .. (386,221.4) -- (386,259.6) .. controls (386,263.13) and (383.13,266) .. (379.6,266) -- (360.4,266) .. controls (356.87,266) and (354,263.13) .. (354,259.6) -- cycle ;
%Shape: Rectangle [id:dp2610722806330268] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ] (357,221.4) -- (383,221.4) -- (383,259.6) -- (357,259.6) -- cycle ;
%Rounded Rect [id:dp018452198608421844] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ] (405,78.4) .. controls (405,74.87) and (407.87,72) .. (411.4,72) -- (430.6,72) .. controls (434.13,72) and (437,74.87) .. (437,78.4) -- (437,116.6) .. controls (437,120.13) and (434.13,123) .. (430.6,123) -- (411.4,123) .. controls (407.87,123) and (405,120.13) .. (405,116.6) -- cycle ;
%Shape: Rectangle [id:dp3503267606845468] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ] (408,78.4) -- (434,78.4) -- (434,116.6) -- (408,116.6) -- cycle ;
%Rounded Rect [id:dp22116465862733725] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ] (454,91.4) .. controls (454,87.87) and (456.87,85) .. (460.4,85) -- (479.6,85) .. controls (483.13,85) and (486,87.87) .. (486,91.4) -- (486,129.6) .. controls (486,133.13) and (483.13,136) .. (479.6,136) -- (460.4,136) .. controls (456.87,136) and (454,133.13) .. (454,129.6) -- cycle ;
%Shape: Rectangle [id:dp9996015319018028] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ] (457,91.4) -- (483,91.4) -- (483,129.6) -- (457,129.6) -- cycle ;
%Rounded Rect [id:dp10774378696214915] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ] (419,139.4) .. controls (419,135.87) and (421.87,133) .. (425.4,133) -- (444.6,133) .. controls (448.13,133) and (451,135.87) .. (451,139.4) -- (451,177.6) .. controls (451,181.13) and (448.13,184) .. (444.6,184) -- (425.4,184) .. controls (421.87,184) and (419,181.13) .. (419,177.6) -- cycle ;
%Shape: Rectangle [id:dp3750016372905083] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ] (422,139.4) -- (448,139.4) -- (448,177.6) -- (422,177.6) -- cycle ;
%Rounded Rect [id:dp6698569940641905] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.3 ] (230,74) .. controls (230,69.58) and (233.58,66) .. (238,66) -- (268,66) .. controls (272.42,66) and (276,69.58) .. (276,74) -- (276,98) .. controls (276,102.42) and (272.42,106) .. (268,106) -- (238,106) .. controls (233.58,106) and (230,102.42) .. (230,98) -- cycle ;
%Curve Lines [id:da18168171902203967] 
\draw    (102,113) .. controls (102,129.66) and (213.41,141.52) .. (240.45,148.57) ;
\draw [shift={(242,149)}, rotate = 196.26] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp6529714522995136] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.3 ] (359,229) .. controls (359,227.34) and (360.34,226) .. (362,226) -- (378,226) .. controls (379.66,226) and (381,227.34) .. (381,229) -- (381,238) .. controls (381,239.66) and (379.66,241) .. (378,241) -- (362,241) .. controls (360.34,241) and (359,239.66) .. (359,238) -- cycle ;
%Straight Lines [id:da4170664338753678] 
\draw    (381,234) -- (406.33,234.31) ;
\draw [shift={(408.33,234.33)}, rotate = 180.7] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp41670436611605366] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ] (410.5,85.7) .. controls (410.5,83.93) and (411.93,82.5) .. (413.7,82.5) -- (428.3,82.5) .. controls (430.07,82.5) and (431.5,83.93) .. (431.5,85.7) -- (431.5,95.3) .. controls (431.5,97.07) and (430.07,98.5) .. (428.3,98.5) -- (413.7,98.5) .. controls (411.93,98.5) and (410.5,97.07) .. (410.5,95.3) -- cycle ;
%Rounded Rect [id:dp4161122351822395] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ] (459.5,98.7) .. controls (459.5,96.93) and (460.93,95.5) .. (462.7,95.5) -- (477.3,95.5) .. controls (479.07,95.5) and (480.5,96.93) .. (480.5,98.7) -- (480.5,108.3) .. controls (480.5,110.07) and (479.07,111.5) .. (477.3,111.5) -- (462.7,111.5) .. controls (460.93,111.5) and (459.5,110.07) .. (459.5,108.3) -- cycle ;
%Rounded Rect [id:dp6150812915155415] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ] (424.5,147.7) .. controls (424.5,145.93) and (425.93,144.5) .. (427.7,144.5) -- (442.3,144.5) .. controls (444.07,144.5) and (445.5,145.93) .. (445.5,147.7) -- (445.5,157.3) .. controls (445.5,159.07) and (444.07,160.5) .. (442.3,160.5) -- (427.7,160.5) .. controls (425.93,160.5) and (424.5,159.07) .. (424.5,157.3) -- cycle ;
%Curve Lines [id:da27281559801222] 
\draw    (283,181) .. controls (326.5,182.5) and (346,208) .. (362,226) ;
%Straight Lines [id:da8983713855112414] 
\draw    (378,241) -- (386.14,251.05) ;
\draw [shift={(387.4,252.6)}, rotate = 230.98] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da2626912041267011] 
\draw    (326.33,233.33) -- (356.67,233.65) ;
\draw [shift={(358.67,233.67)}, rotate = 180.59] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (426,49) node [anchor=north west][inner sep=0.75pt]   [align=left] {MT};
% Text Node
\draw (325,123) node [anchor=north west][inner sep=0.75pt]   [align=left] %{$\mbH_{n,\text{UL}}$};
{$\mathcal{H}^{\text{UL}}$};
% Text Node
\draw (168,116) node [anchor=north west][inner sep=0.75pt]   [align=left] {learn CNN};
% Text Node
\draw (238,174) node [anchor=north west][inner sep=0.75pt]   [align=left] {CNN};
% Text Node
\draw (296,63) node [anchor=north west][inner sep=0.75pt]   [align=left] {collect UL data};
% Text Node
\draw (95,77) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\mathcal{H}$};
% Text Node
\draw (150,61.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {construct train data set};
% Text Node
\draw (242,78) node [anchor=north west][inner sep=0.75pt]   [align=left] {BS};
% Text Node
\draw (361,231.6) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {CNN};
% Text Node
\draw (412.67,228.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {estimated channel ${\mbH}$};
% Text Node
\draw (292.79,155.97) node [anchor=north west][inner sep=0.75pt]  [rotate=-27.38] [align=left] {share parameters};
% Text Node
\draw (240.17,228.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {observation $\mbY$};


\end{tikzpicture}
}
